The role of atmospheric outflows in the migration of hot Jupiters

Many of observed hot Jupiters are subject to atmospheric outflows. Numerical simulations have shown that the matter escaping from the atmosphere can accumulate outside the orbit of the planet, forming a torus. In a few 10^8 yr, the mass of the torus can become large enough to exert a significant gravitational effect on the planet. Accumulation of mass, in its own turn, is hindered by the activity of the star, which leads to the photoevaporation of the torus matter. We explore the role of these and other factors in the planet's migration in the epoch when the protoplanetary disk has already disappeared. Using HD209458 system as an example, we show that the gravitational interaction with the torus leads to the possibility of migration of the planet to its observable position, starting from an orbit >= 0.3 AU.

==> Makefile <==

SRC := paper
OUT := paper_v3.0


$(SRC).pdf: $(SRC).tex
	latexmk -pdf $(SRC)


.PHONY: zip
zip:
	zip $(OUT).zip Makefile *.eps *.pdf *.tex *.sty *.cls


.PHONY: clean
clean:
	rm -f *.log *~ \
		$(addprefix $(SRC),.dvi .ps .pdf .aux .log .fdb_latexmk .fls .out .toc)

